Understanding The Robustness of Self-supervised Learning Through Topic Modeling

Self-supervised learning has significantly improved the performance of many NLP tasks. However, how can self-supervised learning discover useful representations, and why is it better than traditional approaches such as probabilistic models are still largely unknown. In this paper, we focus on the context of topic modeling and highlight a key advantage of self-supervised learning - when applied to data generated by topic models, self-supervised learning can be oblivious to the specific model, and hence is less susceptible to model misspecification. In particular, we prove that commonly used self-supervised objectives based on reconstruction or contrastive samples can both recover useful posterior information for general topic models. Empirically, we show that the same objectives can perform on par with posterior inference using the correct model, while outperforming posterior inference using misspecified models.

==> ssl-topic model/contrastive.tex <==
\section{Guarantees for the Contrastive Objective}\label{sec:contrast}


In this section, we consider the contrastive objective \eqref{eq:constrastive_obj} for self-supervised learning and provide similar provable guarantees on its performance as the reconstruction-based objective.


We use the same approach as \cite{tosh2020contrastive} to construct a representation $g(x)$. 
Given a set of landmark documents $\{l_i\}_{i=1}^m$ with length $|l_i|=t$ as references, the representation is defined as 
\begin{equation}\label{eq:contrast_repr}
\begin{aligned}
    g(x,\{l_i\}_{i=1}^m)=\left(g(x,l_1),\ldots,g(x,l_m)\right)^\top,\quad
    g(x,\xp) = \frac{f(x,\xp)}{1-f(x,\xp)}.    
\end{aligned}
\end{equation}


The following theorem gives the theoretical guarantee for this representation. Similar to Theorem~\ref{thm:reconst_main} for reconstruction-based objective, it shows that any polynomial $P(w)$ of degree at most $t$ can be represented by a linear function of the learned representation. Our proof here relies on the observation that having $g(x,\{l_i\}_{i=1}^m)$ for all short landmark documents of length $t$ gives similar information as $f$ in the reconstruction-based objective does. This observation allows us to remove the anchor words assumption needed in \citep{tosh2020contrastive}.

\begin{restatable}{theorem}{thmcontrastmain}\label{thm:contrast_main}
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose topic-word matrix $A$ satisfies $\rank(A)=K$ and function $f$ minimizes the contrastive objective \eqref{eq:constrastive_obj}. Assume we randomly sampled $m=K^t$ different landmark documents $\{l_i\}_{i=1}^m$ and construct $g(x,\{l_i\}_{i=1}^m)$ as \eqref{eq:contrast_repr}. Then, for any document $x$ and its posterior $w|(x,A)$, the posterior mean of any polynomial $P(w)$ with degree at most $t$ is linear in $g(x,\{l_i\}_{i=1}^m)$. That is, there exists $\theta\in\mathbb{R}^{m}$ such that for all documents $x$
\[
    \E_w[P(w)|x,A] = \theta^\top g(x,\{l_i\}_{i=1}^m).
\]
\end{restatable}


In fact, one can use the same set of documents for both representation and downstream task so that we do not need additional landmark documents. 




==> ssl-topic model/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ssl-topic model/pf_contrastive.tex <==
\newpage
\section{Omitted Proofs in Section~\ref{sec:contrast}}\label{sec:pf_contrast}
In this section, we give the omitted proofs in Section~\ref{sec:contrast}. We give the proof of Theorem~\ref{thm:contrast_main} in Section~\ref{subsec:pf_contrast_main} and proof of Lemma~\ref{lem:contrast_repr} in Section~\ref{subsec:pf_contrast_repr}.


\subsection{Proof of Theorem~\ref{thm:contrast_main}}\label{subsec:pf_contrast_main}
Before presenting the proof of Theorem~\ref{thm:contrast_main}, we first give a characterization of the representation $g(x,\xp)$, which would be useful in the later analysis. Note that this the same as the one shown in \cite{tosh2020contrastive}. We provide its proof for completeness in Section~\ref{subsec:pf_contrast_repr}.
\begin{restatable}{lemma}{lemcontrastrepr}\label{lem:contrast_repr}
If $f$ minimizes the contrastive objective \eqref{eq:constrastive_obj}, then we have
\[
    g(x,\xp)\triangleq\frac{f(x,\xp)}{1-f(x,\xp)} = \frac{\Prob(y=1|x,\xp)}{\Prob(y=0|x,\xp)}.
\]
\end{restatable}

Now we are ready to proof Theorem~\ref{thm:contrast_main}.
\thmcontrastmain*

\begin{proof}
    Since $f$ is the minimizer of contrastive objective \eqref{eq:constrastive_obj}, by Lemma~\ref{lem:contrast_repr} we know
    \[
        g(x,\xp) = \frac{\Prob(y=1|x,\xp)}{\Prob(y=0|x,\xp)}.
    \]
    
    Similar to the proof of Theorem~\ref{thm:reconst_main}, we will show that $g(x,\xp)$ is linear in the topic posterior when $\xp$ is fixed. By Bayes' rule, we have
    \begin{align*}
        g(x,\xp) = \frac{\Prob(x,\xp|y=1)\Prob(y=1)/\Prob(x,\xp)}{\Prob(x,\xp|y=0)\Prob(y=0)/\Prob(x,\xp)}
        = \frac{\Prob(x,\xp|y=1)}{\Prob(x,\xp|y=0)},
    \end{align*}
    where we use $\Prob(y=0)=\Prob(y=1)=1/2$.
    
    Denote the $t$ words in $\xp$ as $\xp_1,\ldots,\xp_t$ and their corresponding topics as $z_1,\ldots,z_t$.
    Then, by our way of generating $x,\xp$, we know
    \begin{align*}
        \Prob(x,\xp|y=0) &= \Prob(x)\Prob(\xp),\\
        \Prob(x,\xp|y=1)
        &= \int_{w} \Prob(\xp_1,\ldots,\xp_t|w,x,y=1)\Prob(w,x|y=1)\rd w\\
        &= \int_{w} \sum_{z_1,\ldots,z_t\in[K]}\Prob(\xp_1,\ldots,\xp_t|z_1,\ldots,z_t,w)\Prob(z_1,\ldots,z_t|w)\Prob(w,x)\rd w,
    \end{align*}
    which implies
    \[g(x,\xp)= \frac{1}{\Prob(\xp)}\int_{w} \sum_{z_1,\ldots,z_t\in[K]}\Prob(\xp_1,\ldots,\xp_t|z_1,\ldots,z_t)\Prob(z_1,\ldots,z_t|w)\Prob(w|x)\rd w\]
    
    Note that
    \begin{align*}
        \Prob(\xp_1,\ldots,\xp_t|z_1,\ldots,z_t)
        =\prod_{i=1}^t \Prob(\xp_i|z_i)
        =\prod_{i=1}^t A_{\xp_1,z_i},
    \end{align*}
    where $A$ is the topic-word matrix. Hence,
    \begin{align*}
        g(x,\xp) 
        &= \frac{1}{\Prob(\xp)}\sum_{z_1,\ldots,z_t\in[K]}\prod_{i=1}^t A_{\xp_1,z_i}\int_{w} \Prob(z_1,\ldots,z_t|w)\Prob(w|x)\rd w\\
        &= \frac{1}{\Prob(\xp)}\sum_{z_1,\ldots,z_t\in[K]}\prod_{i=1}^t A_{\xp_1,z_i}\int_{w} \prod_{i=1}^t w_{z_i}\Prob(w|x)\rd w\\
        &= \frac{1}{\Prob(\xp)}\sum_{z_1,\ldots,z_t\in[K]}\prod_{i=1}^t A_{\xp_1,z_i} \E_w\left[\prod_{i=1}^t w_{z_i}\bigg\vert x\right].
    \end{align*}
    Recall that the topic posterior tensor is $W_{post}=\E_w[w^{\otimes t}|x]\in \mathbb{R}^{K\times \ldots\times K}$, where each entry $[W_{post}]_{z_1,\ldots,z_k}=\E_w[w_{z_1}\ldots w_{z_t}|x]$. Therefore, 
    \begin{align*}
        g(x,\xp)
        &= \frac{1}{\Prob(\xp)}\sum_{z_1, z_2, ...z_t \in [K]} \prod_{i=1}^{t} A_{\xp_i,z_i} [{W_{post}}]_{z_1, z_2, ..., z_t}\\
        &= \frac{1}{\Prob(\xp)}\gA[\xp]^\top \vect(W_{post}),
    \end{align*}
where $\gA = A\otimes A \otimes\cdots\otimes A\in\mathbb{R}^{V^t\times K^t}$, $\gA[\xp]\in\mathbb{R}^{K^t}$ is the row of $\gA$ that correspond to $\xp_1,\ldots,\xp_t$, and $\vect(W_{post})\in\mathbb{R}^{K^t}$ is the vectorization of $W_{post}$. 

Recall we have $m$ randomly sampled different documents $\{l_i\}_{i=1}^n$. Denote $D\in\mathbb{R}^{m\times m}$ as a diagonal matrix such that $D_{i,i}=\Prob(l_i)$, and $\tilde{\gA}\in\mathbb{R}^{m\times K^t}$ as a submatrix of $\gA$ such that each row of $\tilde{\gA}$ is $\gA[l_i]$. Since $l_i$ are randomly sampled, so $D_{i,i}>0$. Thus, we know
\begin{align*}
    g(x,\{l_i\}_{i=1}^n) = D^{-1}\tilde{\gA}\vect(W_{post}),
\end{align*}
which implies $\vect(W_{post})=\tilde{\gA}^\dagger D g(x,\{l_i\}_{i=1}^n)$. Note that we need to show $\tilde{\gA}^\dagger$ is well-defined. Since $A$ has full column rank, we know $\gA$ also has full column rank. Thus, the submatrix $\tilde{\gA}$ also has full column rank since $m=K^t$. This implies $\tilde{\gA}^\dagger$ is well-defined.

Since $P(w)$ is a polynomial of degree at most $t$, we know there exists $\beta$ such that $\E_w[P(w)|x]=\beta^\top \vect(W_{post})$.  Thus, let $\theta = D(\tilde{\gA}^\dagger)^\top \beta$, we have 
\[\E_w[P(w)|x] = \beta^\top \vect(W_{post}) = \theta^\top g(x,\{l_i\}_{i=1}^n).\]

\end{proof}


\subsection{Proof of Lemma~\ref{lem:contrast_repr}}\label{subsec:pf_contrast_repr}

\lemcontrastrepr*
\begin{proof}
    Since $f$ is the minimizer of contrastive objective \eqref{eq:constrastive_obj} and 
    \[L_\contrast(f) = \E_{x,\xp,y}\left[(f(x,\xp)-y)^2\right] = \E_{x,\xp}\left[\E_{y|x,\xp}\left[(f(x,\xp)-y)^2\right]\right], \]
    it is easy to see that $f$ is the Bayes optimal predictor $\Prob(y=1|x,\xp)$. Therefore, we know
    \[g(x,\xp) = \frac{\Prob(y=1|x,\xp)}{\Prob(y=0|x,\xp)}.\]
\end{proof}




\subsection{Discussions on the Self-referencing}\label{subsec:kernel}
The following corollary shows that solving the downstream task is equivalent to solve a kernel regression (in some sense the landmark documents are just random features for this kernel \citep{rahimi2007random}). 
\begin{corollary}\label{coro:kernel}
Denote $\{(x_i,\tilde{y}_i)\}_{i=1}^m$ as the downstream dataset, where $\tilde{y}_i=\E_w[P(w)|x_i]$ is the target for document $x_i$. If we set landmarks $\{l_i\}_{i=1}^m$ to be $\{x_i\}_{i=1}^m$, then solving the downstream task is equivalent to a kernel regression, that is
\begin{align*}
    \arg\min_{\theta} \sum_{k=1}^m\left(\tilde{y}_k - \theta^\top g(x_k,\{l_i\}_{i=1}^m)\right)^2
    = \arg\min_{\theta} \norm{\tilde{y}-G\theta}^2,
\end{align*}
where $\tilde{y}=(\tilde{y}_1,\ldots,\tilde{y}_m)^\top$ and $G\in \mathbb{R}^{m\times m}$ is a kernel matrix such that $G_{ij}=g(x_i,x_j)$.
\end{corollary}


As discussed in Corollary~\ref{coro:kernel}, we show that one can use the same set of documents for both representation and downstream task. Recall that in Theorem~\ref{thm:contrast_main} we need a large number of landmark documents to generate the representation and then use it for the downstream task (e.g., fit a polynomial of topic posterior). However, one may not have enough additional documents to be used as landmarks. Therefore, the benefit of the self-referencing is that we do not need additional landmark documents to generate the representation.

The key observation in Corollary~\ref{coro:kernel} is that the learned representation $g(x,\xp)$ can be viewed as a kernel. Suppose the documents for the downstream task are $x_1,\ldots,x_m$. Construct a kernel matrix $G\in \mathbb{R}^{m\times m}$ such that $G_{ij}=g(x_i,x_j)$. Then, it is easy to see
\[
    \theta^\top g(x_i,\{x_j\}_{j=1}^m) = \theta^\top G_i,
\]
where $G_i$ is the $i$-th column of $G$. Thus,
$\theta$ can be found by the following kernel regression:
\[
    \min_{\theta} \norm{\tilde{y}-G\theta}^2,
\]
where $\tilde{y}=(\tilde{y}_1,\ldots,\tilde{y}_m)^\top$ and $\tilde{y}_i=\E_w[P(w)|x_i]$.



==> ssl-topic model/pf_recovery.tex <==
\section{Omitted Proofs in Section~\ref{sec:reconst}}\label{sec:pf_reconst}

In this section, we give the omitted proofs in Section~\ref{sec:reconst}. We first give a warmup example to illustrate our proof idea in Section~\ref{subsec:reconst_warmup}. Then we give the proof of our main result (Theorem~\ref{thm:reconst_main}) in Section~\ref{subsec:pf_reconst_main} and the proof of robust version (Theorem~\ref{thm:reconst_robust}) in Section~\ref{subsec:pf_reconst_robust}.


\subsection{Warm-Up Example: reconstruct the unknown word}\label{subsec:reconst_warmup}
In this warm-up example, we consider the simple setting where we try to predict the only one unknown word of the document using reconstruction-based objective \eqref{eq:reconstruct_obj}. The following result is the special case of Theorem~\ref{thm:reconst_main} with $t=1$, which shows that the learned representation is able to give any linear function of the topic posterior.

\begin{theorem}\label{thm:reconst_warmup}
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose topic-word matrix $A$ satisfies $\rank(A)=K$ and function $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}. Then, for any document $x$ and its posterior $w|(x,A)$, any linear function $P(w)$ is linear in $f(x)$, that is for any $P(w)=\beta^\top w$, there exists a $\theta\in\mathbb{R}^V$ such that for all documents $x$
\[
    \E_w\left[\beta^\top w|x\right] = \theta^\top f(x).
\] 
\end{theorem}

Following the proof idea described in Section~\ref{sec:reconst}, we first give a characterization of the optimal function $f$. The following lemma shows that $f(x)$ must be the word posterior vector given the document $x$. The proof of this lemma is simply based on the property of the cross-entropy loss function and we defer it to Section~\ref{subsec:pf_reconst_repr_f}. Recall that our vocabulary set is $\gV=\{v_1,\ldots,v_V\}$ and $x_\unsup=(x,y)$ is the given document, where $x$ is unmasked part and $y$ is word marked as unknown. 

\begin{lemma}\label{lem:reconst_repr_f}
If $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}, then we have for all document $x$
\[
    f(x) = \left(\Prob(y=v_1|x),\ldots,\Prob(y=v_V|x)\right)^\top.
\]
\end{lemma}

Based on the above lemma, we are able to prove Theorem \ref{thm:reconst_warmup}. It is easy to see that the word posterior distribution is $A\E_w[w|x]$, so we have $f(x) = A \E_w[w|x]$. Since the columns of $A$ are linearly independent, we know $\E_w[w|x] = A^\dagger f(x)$. Thus, for any linear function $\beta^\top w$, there exists $\theta = (A^\dag)^\top \beta$ such that $\E_w[\beta^\top w|x] = \theta^\top f(x)$. The formal proof of the general case is given in Section~\ref{subsec:pf_reconst_main}.





\subsubsection{Proof of Lemma~\ref{lem:reconst_repr_f}}\label{subsec:pf_reconst_repr_f}
Instead of focusing on the $t=1$ case, we directly give the corresponding lemma of Lemma~\ref{lem:reconst_repr_f} for general $t$. Recall that $x_\unsup=(x,y)$ is the given document, $x$ is the unmasked part, $y=(y_1,\ldots,y_t)$ is the $t$ unknown words that we want to predict and $\gV=\{v_1,\ldots,v_V\}$ is the set of vocabulary. It shows that the optimal $f$ is the $t$ words posterior distribution. Note that the words posterior distribution is linear in the topic posterior of $t$-th moment, which is useful for the later analysis.
\begin{lemma}[Lemma~\ref{lem:reconst_repr_f}, General Case]\label{lem:reconst_repr_f_general}
If $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}, then we have for all document $x$
\[
    f(x) = \left(\Prob(y=(v_1,v_1,\ldots,v_1)|x),\Prob(y=(v_2,v_1,\ldots,v_1)|x),\ldots,\Prob(y=(v_V,v_V,\ldots,v_V)|x)\right)^\top.
\]
\end{lemma}

\begin{proof}
Denote the word posterior distribution as $p^*(x)$. We will show $f(x)=p^*(x)$. By the law of total expectation, we have
\begin{align*}
    L_\reconst = \E_{x,y}[\ell(f(x),y)]
    = \E_x[\E_{y|x}[\ell(f(x),y)|x]].
\end{align*}
We know the probability of $y$ given $x$ is $p^*(x)$. Since $\ell$ is cross-entropy loss, we have
\begin{align*}
    L_\reconst \ge \E_x\left[ -\sum_{k\in[V^t]} [p^*(x)]_k \log [p^*(x)]_k\right],
\end{align*}
where the equality is obtained when $f(x)=p^*(x)$. Thus, when $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}, we have $f(x)=p^*(x)$.
\end{proof}




\subsection{Proof of Theorem~\ref{thm:reconst_main}}\label{subsec:pf_reconst_main}
In this section, we give the proof of Theorem~\ref{thm:reconst_main}.  Theorem~\ref{thm:reconst_warmup} is covered by Theorem~\ref{thm:reconst_main} as the special case of $t=1$. The proof follows the same idea as for Theorem~\ref{thm:reconst_warmup}. We first show that $f(x)$ is the $t$-words posterior (Lemma~\ref{lem:reconst_repr_f_general}). Then just as $t=1$ case where we can recover topic posterior with $A^\dagger f(x)$, we can also recover topic posterior of $t$-th moment with $\gA^\dagger f(x)$ with some matrix $\gA$. The result follows by the observation that for a polynomial $P(w)$ with degree at most $t$, $\E_w[P(w)|x]$ is a linear function of the topic posterior of $t$-th moment.

\thmreconstmain*

\begin{proof} 
Since $f$ is the minimizer of reconstruction-based objective \eqref{eq:reconstruct_obj}, by Lemma~\ref{lem:reconst_repr_f_general} we know given an input document $x$,
\[
    f(x) = \left(\Prob(y
    =(v_1,v_1,\ldots,v_1)|x),\Prob(y=(v_2,v_1,\ldots,v_1)|x),\ldots,\Prob(y=(v_V,v_V,\ldots,v_V)|x)\right)^\top.
\]

We will show that $f(x)$ is linear in the topic posterior. In the following, we focus on $[f(x)]_{y_1,\ldots,y_t}$, which is word posterior probability of the $t$ unknown words being $y_1,\ldots,y_t \in \gV$ given document $x$. Recall $\gS_K$ be the $K-1$ dimensional probability simplex. By the law of total probability, we have
\begin{align*}
    [f(x)]_{y_1,y_2,\ldots,y_t}
    &=\Prob(y_1,y_2,\ldots,y_t|x)\\
    &=\int_{w\in \gS_K} \Prob(y_1,y_2,\ldots,y_t,w|x)\rd w\\
    &=\int_{w\in\gS_K} \Prob(y_1,y_2,\ldots,y_t|w,x)  \Prob(w|x) \rd w\\
    &=\int_{w\in\gS_K} \sum_{z_1,\ldots,z_t \in [K]} \Prob(y_1,y_2,\ldots,y_t, z_1, z_2, ...z_t|w) \Prob(w|x) \rd w\\
    &=\int_{w\in\gS_K} \sum_{z_1,\ldots,z_t \in [K]} \Prob(z_1,,\ldots, z_t|w)\Prob(y_1,\ldots,y_t|z_1,\ldots,z_t,w) \Prob(w|x) \rd w.
\end{align*}

Note that $z_i$ is the topic of word $y_i$. Since we consider the general topic model as Definition~\ref{def:topic_model}, we know 
\[
\Prob(y_1,y_2,\ldots,y_t|z_1, z_2, ..., z_t,w) 
= \Prob(y_1,y_2,\ldots,y_t|z_1, z_2, ..., z_t)
= \prod_{i=1}^t \Prob(y_i|z_i) = \prod_{i=1}^t A_{y_i,z_i},
\]
where $A$ is the topic-word matrix. Hence,
\begin{align*}
    [f(x)]_{y_1,y_2,\ldots,y_t}
    &= \sum_{z_1, z_2, ...z_t \in [K]} \prod_{i=1}^{t} A_{y_i,z_i} \int_{w \in \gS_K}  \Prob(z_1, z_2, ..., z_t|w) \Prob(w|x) \rd w\\
    &= \sum_{z_1, z_2, ...z_t \in [K]} \prod_{i=1}^{t} A_{y_i,z_i} \int_{w \in \gS_K}  \prod_{i=1}^t w_{z_i} \Prob(w|x) \rd w\\
    &= \sum_{z_1, z_2, ...z_t \in [K]} \prod_{i=1}^{t} A_{x_{m+i},z_i} \E_w\left[\prod_{i=1}^t w_{z_i}\bigg\vert x\right].
\end{align*}
Recall that the topic posterior tensor is $W_{post}=\E_w[w^{\otimes t}|x]\in \mathbb{R}^{K\times \ldots\times K}$, where each entry $[W_{post}]_{z_1,\ldots,z_k}=\Prob(z_i\text{ is the topic of word }y_i\text{ for }i\in[t]|x)=\E_w[w_{z_1}\ldots w_{z_t}|x]$. Therefore, 
\begin{align*}
    [f(x)]_{y_1,y_2,\ldots,y_t}
    &= \sum_{z_1, z_2, ...z_t \in [K]} \prod_{i=1}^{t} A_{y_i,z_i} [{W_{post}}]_{z_1, z_2, ..., z_t},\\
    f(x) 
    &= (\underbrace{A\otimes A \otimes\cdots\otimes A}_{t\text{ times}}) \vect(W_{post}),
\end{align*}
where $\otimes$ is the Kronecker product, $\gA = A\otimes A \otimes\cdots\otimes A\in\mathbb{R}^{V^t\times K^t}$ and $\vect(W_{post})\in\mathbb{R}^{K^t}$ is the vectorization of $W_{post}$. Note that $\gA^\dagger = A^\dagger\otimes\cdots\otimes A^\dagger$, so we have $\vect(W_{post})=\gA^\dagger f(x)$.

Since $P(w)$ is a polynomial of degree at most $t$, we know there exists $\beta$ such that $\E_w[P(w)|x]=\beta^\top \vect(W_{post})$.  Thus, let $\theta = (\gA^\dagger)^\top \beta$, we have $\E_w[P(w)|x] = \beta^\top \vect(W_{post}) = \theta^\top f(x)$.
\end{proof}






\subsection{Proof of Theorem~\ref{thm:reconst_robust}}\label{subsec:pf_reconst_robust}

Similar to Lemma~\ref{lem:reconst_repr_f}, we can show that the representation $f(x)$ is close to $t$ words posterior. Then, the key lemma to obtain Theorem~\ref{thm:reconst_robust} is the following result. It suggests that if function $f$ is $\epsilon$-close to the optimal function $f^*$ (word posterior distribution) under cross-entropy loss, then we can still recover the topic posterior with proper $B$ up to $O(\sqrt{\epsilon})$ error. For example, we will choose $B=A^\dagger$ when $t=1$. See the proof of Theorem~\ref{thm:reconst_robust} for the choice of $B$ in the general case.

\begin{restatable}{lemma}{lemreconsterror} \label{lem:reconst_error}
For cross-entropy loss $\ell$ and any two probability vectors $p,p^*$, if $\ell(p,p^*)\le \min_{p:\sum_i p_i=1,p\ge 0}\ell(p,p^*) + \epsilon$, then for any matrix $B$ we have $\norm{B p-B p^*}_1\le \kappa(B)\sqrt{2\epsilon}$.
\end{restatable}

\begin{proof}
Recall that $\ell$ is cross-entropy loss, we know 
\[\ell(p,p^*)-\min_{p:\sum_i p_i=1,p\ge 0}\ell(p,p^*)=\kl{p}{p^*}\le\epsilon.\]
By Pinsker's Inequality, we have that 
\[\norm{p-p^*}_{1}\le \sqrt{2\kl{p^*}{p}}\le \sqrt{2\epsilon}.\]
Then, for any matrix $B$ we have
\begin{align*}
    \norm{B p-B p^*}_1
    \le\kappa(B)||p-p^*||_{1}
    \le\kappa(B)\sqrt{2\epsilon},
\end{align*}
where we use the definition of $\ell_1$ condition number (Definition~\ref{def:l1_cond_num}).
\end{proof}

We now are ready to give the proof of Theorem~\ref{thm:reconst_robust}, which is based on Lemma~\ref{lem:reconst_error} and the proof of Theorem~\ref{thm:reconst_main}.
\thmreconstrobust*

\begin{proof}
Recall from the proof of Theorem~\ref{thm:reconst_main} that $\E_w[P(w)|x] = \beta^\top \vect(W_{post})=\beta^\top \gA^\dagger f^*(x)$, where $\gA^\dagger = A^\dagger\otimes\cdots\otimes A^\dagger$ and $\kappa(\gA^\dagger)=\kappa^t(A^\dagger)$. Same as in the proof of Theorem~\ref{thm:reconst_main}, let $\theta=(\gA^\dagger)^\top \beta$.  We have
\begin{align*}
    \E_x\left[\left( \E_w[P(w)|x] -\theta^\top f(x) \right)^2\right]
    =& \E_x\left[\left( \beta^\top \gA^\dagger f^*(x) -\beta^\top \gA^\dagger  f(x) \right)^2\right]\\
    \le& \E_x\left[\norm{\beta}_2^2 \norm{\gA^\dagger f^*(x) - \gA^\dagger f(x)}_2^2 \right]\\
    \le& \norm{\beta}_2^2\E_x\left[ \norm{\gA^\dagger f^*(x) - \gA^\dagger f(x)}_1^2 \right].
\end{align*}

We are going to use Lemma~\ref{lem:reconst_error} to bound $\norm{\gA^\dagger f^*(x) - \gA^\dagger f(x)}_1$. By Lemma~\ref{lem:reconst_repr_f_general} we know $f^*(x)$ is the word posterior, so $f^*(x)=\E_{y|x}[y|x]$.
Since $\ell$ is cross-entropy loss, we know 
\[
    \E_{y|x}[\ell(f(x),y)-\ell(f^*(x),y)|x]
    =\E_{y|x}\left[\sum_{k\in[V^t]} y_k\log\left(\frac{[f^*(x)]_k}{[f(x)]_k}\right)\bigg\vert x\right]
    =\kl{f^*(x)}{f(x)},
\] 
which implies $\ell(f(x),f^*(x))-\min_{p} \ell(p,f^*(x))\le\epsilon$. Therefore, by Lemma~\ref{lem:reconst_error} with $B=\gA^\dagger$, we know 
\[\norm{\gA^\dagger f(x)-\gA^\dagger f^*(x)}_1\le \kappa(\gA^\dagger)\sqrt{2\epsilon}=\kappa^t(A^\dagger)\sqrt{2\epsilon} .\]

Given the desired bound, we have
\begin{align*}
     \E_x\left[\left( \E_w[P(w)|x] -\theta^\top f(x) \right)^2\right]
    \le& 2\norm{\beta}_2^2 \kappa^{2t}(A^\dagger)\epsilon.
\end{align*}
\end{proof}


\subsection{Discussion on the effective dimension of the representation}\label{subsec:pf_reconst_discussion}

Although the dimension of $f(x)$ is $V^t$, its ``effective dimension" is actually $K^t$, which is much smaller than $V^t$ (the number of topic $K$ usually is much smaller than the size of vocabulary $V$). To see this, let's consider the simple case of $t=1$. As we discussed in the paragraph below Theorem 3.1, we have $f(x)=A\mathbb{E}[w|x,A]$, where $A\in \mathbb{R}^{V \times K}$ is the topic-word matrix and $\mathbb{E}[w|x,A]$ is the posterior mean of $w\in\mathbb{R}^K$. In words, this means that $f(x)$ is completely determined by a linear transformation of a $K$-dimensional vector. Therefore, when we consider the feature of $n$ documents as a matrix $[f(x^{(1)}),...,f(x^{(n)})]\in\mathbb{R}^{V\times n}$, the rank of this matrix is at most $K$ and one can get these $K$-dimensional features by running standard dimension reduction method (e.g., SVD) on the original feature matrix.





==> ssl-topic model/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

In this section we first introduce some general notations. Then we briefly describe the topic models we consider in Section~\ref{subsec:prelim_topic}. Finally we define the self-supervised learning objectives in Section~\ref{subsec:prelim_ssl} and give our main results.

\textbf{Notation }
We use $[n]$ to denote set $\{1,2,\ldots,n\}$. For vector $x\in\mathbb{R}^d$, denote $\norm{x}$ as its $\ell_2$ norm and $\norm{x}_1$ as its $\ell_1$ norm. For matrix $A\in\mathbb{R}^{m\times n}$, we use $A_i\in\mathbb{R}^m$ to denote its $i$-th column. When matrix $A$ has full column rank, denote its left pseudo-inverse as $A^\dagger=(A^\top A)^{-1}A^\top$. For matrix or general tensor $T\in\mathbb{R}^{d_1\times\cdots\times d_l}$, we use vector $\vect(T)\in\mathbb{R}^{d_1\cdots d_l}$ to represent its vectorization. Let $\gS_k=\{x\in\R^k|\sum_{i=1}^k x_i=1, x_i\ge 0\}$ to denote $k-1$ dimensional probability simplex. For two probability vectors $p,q$, define their total variation (TV) distance as $\tv(p,q)=\norm{p-q}_1/2$.


\subsection{Topic Models}
\label{subsec:prelim_topic}

Many topic models treat documents as a bag-of-words and use a two-step procedure of generating a document: first each document is viewed as a probability distribution of topics (often called the topic proportions $w$), and each topic is viewed as a probability distribution over words. To generate a word, one first selects a topic based on the topic proportions $w$, and then samples a word from that particular topic. 
Since the topic distributions are shared across the entire corpus, and the topic proportion vector $w$ is specific to documents, it makes sense to define $w$ as the representation for the document.


More precisely,
let $\mathcal{V}$ be a finite vocabulary with size $V$ and $\mathcal{K}$ be a set of $K$ topics, where each topic is a distribution over $\mathcal{V}$. We denote the topic-word matrix as $A$ with $A_{ij} = \Prob(\text{word}\ i \ |\ \text{topic}\ j)$, so that each column in $A$ represents the word distribution of a topic. Each document corresponds to a convex combination of different topics with proportions $w$. 
For each word in the document, first sample a topic $z$ according to the topic proportions $w$, and then sample the word from the corresponding topic (equivalently, one can also sample a word from distribution $Aw$). Different topic models differ in how they generate $w$, which we formulate in the following definition:

\begin{definition}[General Topic Model]\label{def:topic_model}
A general topic model specifies a distribution $\Delta(K)$ for each number of topics $K$. Given a topic-word matrix $A$ and $\Delta(K)$, to generate a document, one first sample $w\sim \Delta(K)$ and then sample each word in the document from the distribution $Aw$.
\end{definition}

Here $\Delta(K)$ is a prior distribution of $w$ which is crucial when trying to infer the true topic proportions $w$ given the words in a document. Of course, different topic models may also specify different priors for the topic-word matrix $A$. However, given a large number of documents generated from the topic model, in many settings one can hope to learn the topic-word matrix $A$ and the prior distribution $\Delta(K)$ (see e.g., \citet{arora2012learning,arora2016computing}), 
therefore we consider the following inference problem:

\begin{definition}[Topic Inference] Given a topic-word matrix $A$, prior distribution $\Delta(K)$ for topic proportions $w$, and a document $x$, the topic inference problem tries to compute the posterior distribution $w|(x,A)$ given the prior $w\sim \Delta(K)$. \label{def:topic_inference}
\end{definition}

Note that our general topic model can capture many standard topic models, including pure topic model, LDA, CTM and PAM.

\subsection{Semi-supervised Learning Setup} Our goal is to understand the representation learning aspect of self-supervised learning, where we are given large number of unlabeled documents and a small number of labeled documents. In the unsupervised learning stage, the algorithm only has access to the unlabeled documents, and the goal is to learn a representation (a mapping from documents to a feature vector). In the supervised learning stage, the algorithm would use the labeled documents to train a simple classifier that maps the feature vector to the actual label. We often refer to the unsupervised learning stage as ``feature learning'' and the supervised learning stage as ``downstream application''.

In the theoretical model, we assume that the label $y$ is a simple function of the topic proportions $w$. The goal is to apply self-supervised learning on the unlabeled documents to get a good representation, and then use this representation to predict the label $y$. Of course, if one knows the actual parameters of the model, the best predictor for $y$ would be to first estimate the posterior distribution $w$ and then apply the function that maps $w$ to label $y$. We will show that for functions that are approximable by low degree polynomials self-supervised learning can always provide a good representation.


\subsection{Self-supervised learning}
\label{subsec:prelim_ssl}
In general, self-supervised learning tries to turn unlabeled data into a supervised learning problem by hiding some known information. There are many ways to achieve this goal (see e.g., \cite{liu2021self,jaiswal2021survey}). In this paper, we focus on two different approaches for self-supervised learning: reconstruction-based objective and contrastive objective. We first formally define the objectives and then discuss our corresponding result.

\textbf{Reconstruction-Based Objective }
One common approach of self-supervised learning is to first mask part of the data and then try to find a function $f$ to reconstruct the missing part given the unmasked part of input. This is commonly used for language modeling \citep{devlin2018bert,radford2018improving}. In the context of topic modelling, suppose all the documents are generated from an underlying topic model with $A$ and $\Delta(K)$. Then for any given document $x_\unsup$, since each word is i.i.d. sampled (so that the order of words is not important), we pick $t$ random words from the document and mark them as unknown, then we ask the learner to predict these $t$ words given the remaining words in the document. 
Specifically, we split $x_\unsup$ into $x$ and $y$ where $y$ is the $t$ words that we select and let $x$ 
is the document with these $t$ words removed. We aim to select a predictor $f$ that minimizes the following reconstruction objective:
\begin{equation}
\begin{aligned}\label{eq:reconstruct_obj}
    \min _f L_\reconst(f) \triangleq \mathbb{E}_{x,y}[\ell(f(x),y)],
\end{aligned}
\end{equation}
where $\ell(\hat{y},y)=\sum_k -y_k\log \hat{y}_k$ is the cross entropy loss. Here we slightly abuse the notation to use $y$ as an one-hot vector for $V^t$ classes and $f$ also outputs a probability vector on $\gV^t$. Depending on the context, we will use $y$ to denote either the actual next $t$ words or its corresponding one-hot label.
Now we are ready to present our result for the reconstruction-based objective: 
\begin{theorem}(Informal)\label{thm:reconst_informal}
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose function $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}. Then, any polynomial $P(w)$ of the posterior $w|(x,A)$ with degree at most $t$ can be represented by a linear function of $f(x)$. 
\end{theorem}

The theorem shows that if we want to get basic information about posterior distribution (such as mean, variance), then it suffices to predict a small constant number of words (1 for mean and 2 for variance). See Theorem~\ref{thm:reconst_main} for the formal statement.




\textbf{Contrastive Objective }
Another common approach in self-supervised learning is the contrastive learning \citep{he2020momentum,chen2020simple}. In contrastive learning, the training data is usually a pair of data $(x,\xp)$ with a label $y\in\{0,1\}$, where label 1 means $(x,\xp)$ is a positive sample ($x$ and $\xp$ are similar) and label 0 means $(x,\xp)$ is a negative sample ($x$ and $\xp$ are dissimilar). The task is to find a function $f$ such that it can distinguish the positive sample and negative sample, i.e., $f(x,\xp)=y$. Formally, we want to select a predictor $f$ such that it minimizes the following contrastive objective:
\begin{equation}\label{eq:constrastive_obj}
    \min_{f} L_\contrast\triangleq \mathbb{E}_{x,\xp,y}[\ell(f(x,\xp),y)].    
\end{equation}
In the context of topic models, following previous work \citep{tosh2020contrastive}, we generate the data $(x,\xp,y)$ as follows. Suppose all documents are generated from an underlying topic model with $A$ and $\Delta(K)$. We first generate a document $x$ from the word distribution $Aw$ where $w$ is sampled from $\Delta(K)$. Then, (i) with half probability we generate $t$ words from the same distribution $Aw$ to form the document $\xp$ and set $y=1$; (ii) with half probability we generate $t$ words from a different word distribution $Aw^\prime$ with $w^\prime \sim \Delta(K)$ (so that $w\neq w^\prime$) and set $y=0$. 
We consider the square loss $\ell(\hat{y},y)=(\hat{y}-y)^2$ for simplicity. 

We now give our informal result on contrastive objective. 
See Theorem~\ref{thm:contrast_main} for the formal statement. Note that this theorem generalizes Theorem 3 in \cite{tosh2020contrastive}.

\begin{theorem}(Informal)
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose function $f$ minimizes the contrastive objective \eqref{eq:constrastive_obj}. Then we can use $f$ and enough documents to construct a representation $g(x)$ such that any polynomial $P(w)$ of the posterior $w|(x,A)$ with degree at most $t$ can be represented by a linear function of $g(x)$.
\end{theorem}

\vspace{-0.1in}
\paragraph{Advantage of SSL approach} Note that neither objectives \eqref{eq:reconstruct_obj} or \eqref{eq:constrastive_obj} depend on the prior distribution $\Delta(K)$, so it is possible to optimize these without specifying a specific model; on the other hand, even the definition of topic inference (Definition~\ref{def:topic_inference}) relies heavily on $\Delta(K)$. 




==> ssl-topic model/realdata.tex <==
\section{Experiments on Real Data}\label{sec:real_experiment}

The self-supervised learning approach studied in this paper is simplified for theoretical analysis as it uses a bag-of-words approach.
In this section, we show that although this simplified approach is not state-of-art, it has reasonable performance compared to several baselines. 

\vspace{-0.1in}
\paragraph{Experiment Setup}

We use the AG news dataset \citep{zhang2015character}, in which each document has a label of one out of four categories: world, sports, business, and sci/tech. 
Each category has 30,000 samples in the training set and 19,000 samples in the testing set. The number of words in the vocabulary is about 16,700. We generally follow the experiment setup done by \cite{tosh2020contrastive} (see more details in Section~\ref{subsec:real_data_process}), but the representation we used is generated by our reconstruction-based objective. Experiment results on two additional datasets are provided in Appendix~\ref{sec:more_real_data}. 

Our training follows the semi-supervised setup that involves two major phases: unsupervised phase and supervised phase. In the unsupervised phase, we train the self-supervised model with reconstruction-based objective on most of training data. In the supervised phase, using the document representation generated by the SSL model as input, we train a linear classifier to classify the category of the documents using multi-class logistics regression (by Scikit-learn \citep{scikit-learn}) with 3-fold cross validation for parameter tuning ($l_2$ regularization term and solver). 
We measure the topic recovery accuracy on test set to compare the performance of different methods.


We choose residual blocks as the basic building block for our neural network architecture, with varying width and depth. The network used for Figure~\ref{fig:rep_comp} has 3 residual blocks and a width of 4096 neurons per layer. 
Other detailed hyperparameters and ablation studies can be found in Appendix~\ref{subsec:realdata_model_arch}. 
We train the model using reconstruction-based objective \eqref{eq:reconstruct_obj} with $t= 1$ using the same variance-reduction technique in synthetic experiments. 


To extract our representation, we use an identity matrix to replace the last layer. That is, we take a softmax function on top of the second-to-last layer of the neural network. This is different from our theory but we found that it effectively reduces the high output dimension 
and improves performance. We include more details in Section~\ref{subsec:realdata_rep_extract} in Appendix. 

\vspace{-0.1in}
\paragraph{Experiment Results}


\begin{figure}[t]
    \centering
    \subfigure{\includegraphics[width=0.45\textwidth]{experiment_results/rep_comp_may17_lda.png}}
    \caption{Performances of RBL, NCE and baselines (BOW, Word2vec, LDA) on real data.}
    \label{fig:rep_comp}
\end{figure}



The performance of Reconstruction-Based Learning representation (RBL) is shown in Figure~\ref{fig:rep_comp}, where the test accuracy on representation is plotted against number of training samples used to train the classifier in supervised learning phase. The representation RBL performs better than both bag-of-words (BOW),Word2vec and LDA baselines (see more details about baselines in Section~\ref{subsec:realdata_rep_extract}). Notably, Word2vec representation is inferior only by a small margin, and works well in general even when limited training samples are provided. On the contrary, although BOW representation has a decent test accuracy when training samples are abundant, it performs significantly poorly on smaller training set.  

We also compare our result to previous noise contrastive estimation (NCE) representation benchmark achieved by \cite{tosh2020contrastive} using contrastive objective, where their reported best accuracy is around $87.5\%$ when full 4000 training samples are used, slightly higher than our RBL corresponding test accuracy of $87.1\%$. In our attempt to reproduce their result, parameter tuning yields the best accuracy of $86\%$ when full training samples were used. We plot our own reproduced results on in Figure~\ref{fig:rep_comp} since parameter tuning does not achieve a close benchmark to their result.



==> ssl-topic model/recovery.tex <==
\section{Guarantees for the Reconstruction-Based Objective}\label{sec:reconst}

In this section, we consider the reconstruction-based objective \eqref{eq:reconstruct_obj} and provide theoretical guarantees for its performance. We first show that if such objective with $t$ unknown words can be minimized, then any polynomial of topic posterior $w|(x,A)$ with degree at most $t$ can be represented by a linear function of the learned representation.


\begin{restatable}[Main Result]{theorem}{thmreconstmain}\label{thm:reconst_main}
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose topic-word matrix $A$ satisfies $\rank(A)=K$ and function $f$ minimizes the reconstruction-based objective \eqref{eq:reconstruct_obj}. Then, for any document $x$ and its posterior $w|(x,A)$, the posterior mean of any polynomial $P(w)$ with degree at most $t$ is linear in $f(x)$. That is, there exists a $\theta\in\mathbb{R}^{V^t}$ such that for all documents $x$
\[
    \E_w[P(w)|x,A] = \theta^\top f(x).
\]
\end{restatable}

To understand this theorem, first consider a warm-up example where $t=1$ (see details in Section~\ref{subsec:reconst_warmup} in appendix). Intuitively, in this case the best way to predict the missing word for a given document $x$ is to estimate its topic proportion $w$, and then predict the word using $Aw$ where $A$ is the topic-word matrix. Therefore, if the output of self-supervised learning $f(x)$ (which is a $V$-dimensional vector indexed by words) minimizes the loss, then $f(x)$ must have the form $f(x) = A\E[w|x,A]$. When $A$ is full rank multiplying by the pseudo-inverse of $A$ recovers the expectation of the posterior $w|(x,A)$.  
The proof for the general case of predicting $t$-words requires more careful characterization of the optimal prediction and its relationship to $\E_w[P(w)|x,A]$, which we defer to Section~\ref{subsec:pf_reconst_main}.

The above discussion also suggests that though the representation dimension may seem to be $V^t$, its ``effective" dimension is in fact $K^t$ which is much smaller than $V^t$. See more details in Appendix~\ref{subsec:pf_reconst_discussion}.

\vspace{-0.1in}
\paragraph{Robustness for an approximate minimizer}
In Theorem~\ref{thm:reconst_main} we focus on the case when function $f$ is exactly the minimizer of the reconstruction-based objective \eqref{eq:reconstruct_obj}, i.e., $L_\reconst(f)=L_\reconst^*\triangleq\min_f L_\reconst(f)$. However, in practice one cannot hope to find such a function exactly. In the following, we provide a robust version of Theorem~\ref{thm:reconst_main} such that it allows us to find an approximate solution instead of the exact optimal solution.

To present our result, we need to first introduce the following notion of condition number, which was used in many previous works, such as collaborative filtering systems \citep{kleinberg2008using} and topic models \citep{arora2016provable}. Intuitively, $\kappa(B)$ measures how large a vector would change after multiplying with $B$ in the $\ell_1$ norm sense.

\begin{definition}[$\ell_1$ Condition Number]\label{def:l1_cond_num}
For matrix $B\in\mathbb{R}^{m\times n}$, define its $\ell_1$ condition number $\kappa(B)$ as
$\kappa(B)\triangleq\min_{x\in\mathbb{R}^n: x\neq 0} \norm{Bx}_1/\norm{x}_1=\max_{i\in[n]} \norm{B_i}_1,
$
where $B_i$ is the $i$-th column of $B$.
\end{definition}

Let $W_{post}\in\mathbb{R}^{K\times\cdots\times K}$ be the topic posterior tensor for $t$ unknown words $y=(y_1,\ldots,y_t)$ given remaining document $x$. That is, for each entry $[W_{post}]_{z_1,\ldots,z_k}=\Prob( \text{for all $i$, $z_i$ is the topic of word $y_i$}|x,A)=\E_w[w_{z_1}\cdots w_{z_t}|x,A]$ and $W_{post}=\E_w[w^{\otimes t}|x,A]$.\footnote{To simply the notations, WLOG assume topic set $\gK=[K]$ so that we can use topics $z_i\in[K]$ as indices.} Thus, any polynomial $P(w)$ of degree at most $t$ can be represented as $\E_w[P(w)|x,A]=\beta^\top \vect(W_{post})$ for some $\beta$, where $\vect(W_{post})\in\mathbb{R}^{K^t}$ is the vectorization of $W_{post}$.

We now are ready to present the robust version of Theorem~\ref{thm:reconst_main}. It shows if we only find a function $f$ whose loss is at most $\epsilon$ larger than the optimal loss, then a linear transformation of our learned representation can still give a good approximation of the target polynomial within a $O(\epsilon)$ error. 

\begin{restatable}[Robust Version]{theorem}{thmreconstrobust}\label{thm:reconst_robust}
Consider the general topic model setting as Definition \ref{def:topic_model}, suppose topic-word matrix $A$ satisfies $\rank(A)=K$ and function $f$ satisfies $L_\reconst(f)\le L_\reconst^* + \epsilon$ for some $\epsilon>0$. Then, for any document $x$ and its posterior $w|(x,A)$, the posterior mean of any polynomial $P(w)$ with degree at most $t$ is approximately linear in $f(x)$. That is, there exists a $\theta\in\mathbb{R}^{V^t}$ such that
\[
    \E_x\left[\left(\E_w[P(w)|x,A] - \theta^\top f(x)\right)^2\right]\le 2\norm{\beta}^2\kappa^{2t}(A^\dagger) \epsilon,
\]
where $\E_w[P(w)|x,A]=\beta^\top\vect(W_{post})$.
\end{restatable}

Note that the dependency on $\norm{\beta}^2\kappa^{2t}(A^\dagger)$ is expected, since this is the norm $\norm{\theta}^2$ that we would have if $\epsilon=0$, i.e., the $\theta$ we would have in Theorem~\ref{thm:reconst_main}. Thus, this quantity should be understood as the complexity of the target function for the downstream task. Empirically we show that $\kappa(A^\dagger)$ is small in Section~\ref{subsec:cond_num}. 
The proof is deferred to Section~\ref{subsec:pf_reconst_robust}.













==> ssl-topic model/synthetic.tex <==
\vspace{-0.05in}
\section{Synthetic Experiments}\label{sec:syn_experiment}

In this section, we optimize the reconstruction-based objective \eqref{eq:reconstruct_obj} on data generated by several topic models to show that 
self-supervised learning performs on par with inference using correct model, and both of them outperform inference with misspecified models. 


\vspace{-0.05in}
\subsection{Topic Models}
We consider four types of topic models in our experiments. Our first topic model is the pure-topic model, where each document's topic comes from a discrete uniform distribution over the $K$-dimensional linear basis, namely $\{e_1, e_2, ..., e_K\}$. Our second topic model is the Latent Dirichlet Allocation (LDA) model, where $\Delta(K)$ is a symmetric Dirichlet distribution $\dir(1/K)$. 


We are also interested in topic models that involve more subtle topic correlations and similarities between different topic's word distributions. To this end, we consider the Correlated Topic Model (CTM) \citep{blei2007correlated} and the Pachinko Allocation Model (PAM) \citep{li2006pachinko}. Our goal is to construct settings where the correlation between topics provide useful information for inference. To achieve this goal, in CTM, we construct groups of 4 topics. Within the group, topic pairs (0,2) and (1,3) are highly correlated (as specified by the prior), while topics 0 and 1 share many words (see Figure~\ref{fig:topic_dist} for an illustration of the setting). In this case, if we observe a document with words that could either belong to topic 0 or 1, but this same document also has words that are associated with topic 2, we can infer that the first set of words are likely from topic 0, not topic 1.  We construct such correlations in CTM by setting  the diagonal entries of its Gaussian covariance matrix to 15 and the covariance between correlated pairs of topics to 0.99 times the diagonal entries, with the remaining entries set to zero. We construct similar examples for PAM, see Appendix~\ref{sec:more_synthetic} for details.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.32\textwidth]{experiment_results/ctm_topic_dist_4_topics.png}
    \includegraphics[width=0.35\textwidth]{experiment_results/CTM_topic_mat_vis_4_topics.png}
    \caption{One example of a group of 4 topics in the Correlated Topic Model. \textbf{Left:} Weight of each topic in a document's topic proportion. In this example topics 1 and 3 have large proportions as they are correlated. \textbf{Right:} Pairwise topic similarity (cosine similarity of the pair's word distribution). }
    \label{fig:topic_dist}
\end{figure}

\vspace{-0.05in}
\subsection{Simulation Setup}

\vspace{-0.05in}
\paragraph{Document generation} 
Our documents are synthetically generated through the following steps: we first construct a $V\times K$ 
topic-word matrix $A$. Then, for each document, we determine the document length $n$ from Poisson distribution $\pois(\lambda)$, draw a topic distribution $w$ from $\Delta(K)$, and draw $n$ words i.i.d. from the word distribution given by $Aw$. In our simulation, we set $K=20, V=5000, \lambda \in \{30,60\}$.
Often $A$ will be drawn from a Dirichlet distribution $\dir(\alpha/K)$ (see Appendix~\ref{sec:more_synthetic} for details), and we take $\alpha=1,3,5,7,9$ to vary the difficulty level of the inference problem, where a larger $\alpha$ introduces more similarity between topics. 

\vspace{-0.05in}
\paragraph{Neural network models }
We consider two different network architectures as $f$ in the experiments: (1) Fully-connected network with residual connection, with bag-of-words document representation as the input since the order does not matter in topic models; (2) Attention-based architecture. Due to the architecture of attention, the input needs to be a sequence of words instead of bag-of-words vector. Thus, we transform bag-of-words representation into full document by repeating each word by its frequency and concatenating them in random order, and then use the full document as the input. More specifically, the attention-based architecture contains 8 transformer blocks where each transformer block consists of a 768-dimensional attention layer and a feed-forward layer, with residual connection applied around every block. The network's second to last layer averages over the outputs of the last transformer block and the final layer projects it to a $V$-dimensional word distribution. See more details in Section~\ref{subsec:hyperparam}. 
We find that fully-connected neural network with residual connections performs the best on recovering topic posterior distribution for pure-topic and LDA documents, and attention-based architecture \citep{vaswani2017attention} performs the best for recovering topic posterior distribution for CTM and PAM documents. 



\vspace{-0.05in}
\paragraph{Training setup}
During training, we resample 60,000 new documents after every 2 epochs, and the total amount of training data varies from 720K documents to 6M documents. The loss function is the reconstruction-based objective \eqref{eq:reconstruct_obj} with $t=1$, i.e., we want the model to predict one missing word. To reduce the variance during the training, in each training document, we sampled 6 words as the prediction target, hide them from the model and ask the model to predict each word separately. The trained model is evaluated on test documents generated from the same topic prior as the training documents. We use 5,000 test documents for the pure-topic prior and 200 test documents for the remaining priors. For each test document, we use MCMC (see Appendix~\ref{subsec:sampling_details}) assuming the document's correct topic prior to approximate the ground truth topic posterior. To get the posterior estimations from SSL approach, we multiply the pseudo-inverse of the topic matrix $A$ with the model output $f(x)$ to get the estimated posterior mean vector $A^\dag f(x)$ as we explained in Section~\ref{sec:reconst} (and also Section~\ref{subsec:reconst_warmup}). Then, we measure topic posterior recovery loss as the Total Variation (TV) distance between the recovered topic posterior mean vector and the ground truth topic posterior mean vector.


\vspace{-0.04in}
\subsection{Experiment Results}\label{subsec:syn_experiment_result}


\vspace{-0.04in}
\paragraph{Topic posterior recovery } As illustrated in Table~\ref{tab:tv_map}, after 200 training epochs, our model can accurately recover the topic posterior mean vector. 
Meanwhile, it can be observed that for larger values of the Dirichlet hyperparameter $\alpha$, the recovery loss gets higher. This is expected because 
higher $\alpha$ leads to more similar topics, which makes the learning problem more difficult. This effect is also captured by Definition~\ref{def:l1_cond_num} and we show the computed condition numbers in Section~\ref{subsec:cond_num}. 

\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{ccccc}
\hline
\begin{tabular}[c]{@{}c@{}}TV \\ Distance \end{tabular}    & \multicolumn{4}{c}{Document Type}                                                                                                                                                                                  \\
\multicolumn{1}{c}{$\alpha$} & Pure                       & LDA                                                        & CTM                                                        & PAM                                                         \\ \hline
1                         & \begin{tabular}[c]{@{}c@{}} 0.0148 \\± 0.0020 \end{tabular}                    & \begin{tabular}[c]{@{}c@{}}0.0757 \\ ± 0.0033\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0550\\ ± 0.0037\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0.0489 \\ ± 0.0025\end{tabular}  \\ \hline
3                         & \begin{tabular}[c]{@{}c@{}} 0.0308 \\± 0.0076 \end{tabular}                     & \begin{tabular}[c]{@{}c@{}}0.0899 \\ ± 0.0053\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0799 \\ ± 0.0048\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0712 \\ ± 0.0038\end{tabular}  \\ \hline
5                         & \begin{tabular}[c]{@{}c@{}} 0.0501 \\± 0.0030 \end{tabular}                     & \begin{tabular}[c]{@{}c@{}}0.1041 \\ ± 0.0062\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0970 \\ ± 0.0057\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0787 \\ ±  0.0043\end{tabular} \\ \hline
7                         & \begin{tabular}[c]{@{}c@{}} 0.0391 \\± 0.0022 \end{tabular}                     & \begin{tabular}[c]{@{}c@{}}0.1233 \\ ± 0.0071\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1071 \\ ± 0.0068\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0960 \\ ± 0.0057\end{tabular}  \\ \hline
9                         & \begin{tabular}[c]{@{}c@{}} 0.0517 \\± 0.0045 \end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1358 \\ ± 0.0089\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1101 \\ ± 0.0064\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.0971 \\ ± 0.0053\end{tabular}  \\ \hline
\end{tabular}
}
\hspace{0.5cm}
\scalebox{0.6}{
\begin{tabular}{ccccc}
\hline
\begin{tabular}[c]{@{}c@{}}{\tiny Major Topic(s)} \\ {\tiny Recovery Accuracy}\end{tabular} & \multicolumn{4}{c}{Document Type}                                                                                                                                                                                                                \\
$\alpha$                                                              & Pure                                                      & LDA                                                        & CTM                                                        & PAM                                                        \\ \hline
1                                                                  & \begin{tabular}[c]{@{}c@{}}1.0000\\ ± 0.0000\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9050 \\ ± 0.0406\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9175 \\ ± 0.0275\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9025 \\ ± 0.0330\end{tabular} \\ \hline
3                                                                  & \begin{tabular}[c]{@{}c@{}}1.0000\\ ± 0.0000\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8750 \\ ± 0.0458\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8900 \\ ± 0.0311\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8950 \\ ± 0.0344\end{tabular} \\ \hline
5                                                                  & \begin{tabular}[c]{@{}c@{}}1.0000\\ ± 0.0000\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9000 \\ ± 0.0416\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8975 \\ ± 0.0296\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8675 \\ ± 0.0407\end{tabular} \\ \hline
7                                                                  & \begin{tabular}[c]{@{}c@{}}1.0000\\ ± 0.0000\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9150 \\ ± 0.0387\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8675 \\ ± 0.0383\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8675 \\ ± 0.0407\end{tabular} \\ \hline
9                                                                  & \begin{tabular}[c]{@{}c@{}}0.9950\\ ± 0.0098\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.9100 \\ ± 0.0397\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8850 \\ ± 0.0330\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.8325 \\ ± 0.0461\end{tabular} \\ \hline
\end{tabular}
}
\caption{Self-supervised learning approach performs reasonably on recovering the topic posterior mean. \textbf{Left:} TV distance between recovered topic posterior (self-supervised learning approach) and true topic posterior for different topic models. \textbf{Right:} Major topic(s) recovery accuracy for different topic models. The 95\% confidence interval is reported in both tables.}
\label{tab:tv_map}
\end{table}



\vspace{-0.05in}
\paragraph{Major topic recovery } We examine the extent our recovered topic posterior captures the major topics in a given document. For pure-topic and LDA documents, we measure major topic recovery accuracy of correctly estimating the topic with largest proportion. 
Considering that topics in CTM and PAM documents are correlated in pairs, we measure the major topic recovery accuracy for CTM and PAM as the top-2 topic overlap rate on their test documents. Table~\ref{tab:tv_map} shows that our algorithm is successful throughout all settings we consider.


\vspace{-0.05in}
\paragraph{Robustness of self-supervised learning} 
We compare the self-supervised approach to traditional topic inference (MCMC with a specifed topic prior, the results on variational inference are reported in Section~\ref{subsec:tv_map}). 
Specifically, for each $\alpha$ value, we take 200 test documents from each category of documents, and we run posterior inference assuming a specific topic model and calculate the TV distance between this posterior mean vector and the ground truth posterior mean vector. We exclude assuming pure-topic prior from our comparison because it gives invalid results for documents with mixed topics. 
For $\alpha=1$, as shown in Table~\ref{table: tv_ssl_vs_other}, the topic posterior recovered from SSL approach is closer to the ground truth topic posterior than that recovered from a misspecified topic prior. 

We also report the major topic recovery accuracy for SSL approach against topic inference using both correct and incorrect topic model in Table~\ref{table: tv_ssl_vs_other}. The major topic recovery rate of SSL approach is similar to that of posterior inference assuming the correct prior. For pure topic model, all four methods get 100\% major topics recovery rate on pure-topic documents. For LDA, again all four methods perform similarly well since the instance is not difficult. However we observe significant difference for more complicated CTM and PAM models. For these models, the SSL approach performs similarly to posterior inference using the correct model, and both of them are significantly better than posterior inference using misspecified models. The results for $\alpha=3,5,7,9$ are presented in Section~\ref{sec:more_synthetic}. The comparison further reveals the robustness of self-superivised learning. 

\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{lcccc}
\hline
TV Distance & \multicolumn{4}{c}{Document Type ($\alpha=1$)}                                                                                                                                                                                                                \\
Method      & Pure                                                       & LDA                                                        & CTM                                                                 & PAM                                                        \\ \hline
LDA         & \begin{tabular}[c]{@{}c@{}}0.0406 \\ ± 0.0016 \end{tabular}           & -                                                          & \begin{tabular}[c]{@{}c@{}}0.1182 \\ ± 0.0099\end{tabular}          & \begin{tabular}[c]{@{}c@{}}0.1218 \\ ± 0.0096\end{tabular} \\ \hline
CTM         & \begin{tabular}[c]{@{}c@{}} 0.2083 \\ ± 0.0038 \end{tabular}            & \begin{tabular}[c]{@{}c@{}}0.2060 \\ ± 0.0064\end{tabular} & -                                                                   & \begin{tabular}[c]{@{}c@{}}0.3154 \\ ± 0.0082\end{tabular} \\ \hline
PAM         & \begin{tabular}[c]{@{}c@{}} 0.3782 \\ ± 0.0038 \end{tabular}            & \begin{tabular}[c]{@{}c@{}}0.3459 \\ ± 0.0128\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.3939 \\ ± 0.0096\end{tabular}          & -                                                          \\ \hline
\textbf{SSL (ours)}  & \textbf{\begin{tabular}[c]{@{}c@{}} 0.0148 \\ ± 0.0020\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0757 \\ ± 0.0033\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0550 \\ ± 0.0037\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0489 \\ ± 0.0025\end{tabular}} \\ \hline
\end{tabular}
}
\hspace{0.5cm}
\scalebox{0.7}{
\begin{tabular}{lccc}
\hline
Major Topic(s) Recovery & \multicolumn{3}{c}{Document Type ($\alpha=1$)}                                                                                                                                                                     \\
Method                  & LDA                                                                 & CTM                                                                 & PAM                                                                 \\ \hline
LDA                     & \textbf{\begin{tabular}[c]{@{}c@{}}0.9150 \\ ± 0.0387\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.8850 \\ ± 0.0344\end{tabular}          & \begin{tabular}[c]{@{}c@{}}0.8500 \\ ± 0.0360\end{tabular}          \\ \hline
CTM                     & \begin{tabular}[c]{@{}c@{}}0.9000 \\ ± 0.0416\end{tabular}          & \textbf{\begin{tabular}[c]{@{}c@{}}0.9175 \\ ± 0.0275\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.8300 \\ ± 0.0370\end{tabular}          \\ \hline
PAM                     & \begin{tabular}[c]{@{}c@{}}0.8750 \\ ± 0.0458\end{tabular}          & \begin{tabular}[c]{@{}c@{}}0.7250 \\ ± 0.0397\end{tabular}          & \textbf{\begin{tabular}[c]{@{}c@{}}0.9050 \\ ± 0.0320\end{tabular}} \\ \hline
\textbf{SSL (ours)}              & \begin{tabular}[c]{@{}c@{}}0.9050 \\ ± 0.0406\end{tabular}          & \textbf{\begin{tabular}[c]{@{}c@{}}0.9175 \\ ± 0.0275\end{tabular}} & \begin{tabular}[c]{@{}c@{}}0.9025 \\ ± 0.0330\end{tabular}          \\ \hline

\end{tabular}
}


\caption{Robustness of self-supervised learning approach. \textbf{Left:} TV distance between recovered topic posterior and true topic posterior of self-supervised learning approach versus posterior inference via Markov Chain Monte Carlo assuming a specific prior for $\alpha=1$. \textbf{Right:} Major topic recovery rate of our approach versus posterior inference via Markov Chain Monte Carlo assuming a specific prior for $\alpha=1$. In both table, the 95\% confidence interval is reported.}.
\label{table: tv_ssl_vs_other}
\end{table}
